Periodic Materials Generation using Text-Guided Joint Diffusion Model

Equivariant diffusion models have emerged as the prevailing approach for generating novel crystal materials due to their ability to leverage the physical symmetries of periodic material structures. However, current models do not effectively learn the joint distribution of atom types, fractional coordinates, and lattice structure of the crystal material in a cohesive end-to-end diffusion framework. Also, none of these models work under realistic setups, where users specify the desired characteristics that the generated structures must match. In this work, we introduce TGDMat, a novel text-guided diffusion model designed for 3D periodic material generation. Our approach integrates global structural knowledge through textual descriptions at each denoising step while jointly generating atom coordinates, types, and lattice structure using a periodic-E(3)-equivariant graph neural network (GNN). Extensive experiments using popular datasets on benchmark tasks reveal that TGDMat outperforms existing baseline methods by a good margin. Notably, for the structure prediction task, with just one generated sample, TGDMat outperforms all baseline models, highlighting the importance of text-guided diffusion. Further, in the generation task, TGDMat surpasses all baselines and their text-fusion variants, showcasing the effectiveness of the joint diffusion paradigm. Additionally, incorporating textual knowledge reduces overall training and sampling computational overhead while enhancing generative performance when utilizing real-world textual prompts from experts.

==> Sections/tables_figs.tex <==
% TABLE 1 ------------>
\begin{table}
  \centering
    \setlength{\tabcolsep}{2.5 pt}
    \renewcommand{\arraystretch}{1.2}
    \scalebox{0.9}{
    \begin{tabular}{ |c|c|c|c|c|c| }
 \hline
 % Header
 \multirow{2}*{Method} & \multirow{2}*{\# Samples} & \multicolumn{2}{|c|}{Perov-5} & \multicolumn{2}{|c|}{Carbon-24} \\
 \cline{3-6}
  & & Match Rate $\uparrow$ & RMSE $\downarrow$ & Match Rate $\uparrow $& RMSE $\downarrow$ \\
 \hline
 % \hline

  % RS
  \multirow{2}*{RS \cite{cheng2022crystal}} & 20 & 29.22 & 0.2924 & 14.63 & 0.4041 \\
  \cline{2-6}
   & 5,000 & 36.56 & 0.0886 & 14.63 & 0.4041 \\
  \hline

  % BO
  \multirow{2}*{BO \cite{cheng2022crystal}} & 20 & 21.03 & 0.2830 & 0.44 & 0.3653 \\
  \cline{2-6}
   & 5,000 & 55.09 & 0.2037 & 12.17 & 0.4089 \\
  \hline

  % PSO
  \multirow{2}*{PSO \cite{cheng2022crystal}} & 20 & 20.90 & 0.0836 & 6.40 & 0.4204 \\
  \cline{2-6}
   & 5,000 & 21.88 & 0.0844 & 6.50 & 0.4211 \\
  \hline
  % \hline

  % P-cG-SchNet
  \multirow{2}*{P-cG-} & 1 & 48.22 & 0.4179 & 17.29 & 0.3846 \\
  \cline{2-6}
  SchNet \cite{gebauer2022inverse}  & 20 & 97.94 & 0.3463 & 55.91 & 0.3551 \\
  \hline

  % CDVAE
  \multirow{2}*{CDVAE} & 1 & 45.31 & 0.1138 & 17.09 & 0.2969 \\
  \cline{2-6}
   & 20 & 88.51 & 0.0464 & 88.37 & 0.2286 \\
  \hline

   % DiffCSP
   \multirow{2}*{DiffCSP} & 1 & 52.02 \textbf{*} & 0.0760 \textbf{*} & 17.54 \textbf{*} & 0.2759 \textbf{*} \\
  \cline{2-6}
   & 20 & \textbf{98.60} & 0.0128 \textbf{*} & 88.47 \textbf{*} & 0.2192 \textbf{*} \\
  \hline

  % Ours - atom
  \multirow{2}*{\our{}} & 1 & \textbf{95.24} & \textbf{0.0194} & \textbf{53.64} & \textbf{0.1666} \\
  \cline{2-6}
   & 20 & 98.25 \textbf{*} & \textbf{0.0085} & \textbf{97.58} & \textbf{0.1154} \\
  \hline

  % Ours + atom
  % \multirow{2}*{Ours w atom types} & 1 & - & - & - & - & - & - \\
  % \cline{2-8}
  %  & 20 & - & - & - & - & - & - \\
  % \hline

 \end{tabular}
 }
   \caption{The best performance is highlighted in bold.}
  \label{tbl-recons}
\end{table}
% TABLE 1 END ------------>

% TABLE 2 ------------>
\begin{table*}
  \centering
    \setlength{\tabcolsep}{4 pt}
    \renewcommand{\arraystretch}{1}
 % \begin{tabularx}{\textwidth}{ |c|c|X|X|X|X|X|X|X| }
 \scalebox{1}{
 \begin{tabularx}{\textwidth}{ |c|c|c|c|c|c|c|c|c| }
 % \begin{tabularx}{\textwidth}{ |c|c|c|c|c|c|c|c|c| }
  \cline{1-9}
  % Header
  % Comp val on two rows -->
  % \multirow{2}*{Dataset} & \multirow{2}*{Method} & \multicolumn{2}{|c|}{Validity $\uparrow$} & \multicolumn{2}{|c|}{COV $\uparrow$} & \multicolumn{3}{|c|}{Property Statistics $\downarrow$} \\
  % \cline{3-9}
  %  & & Compositional & Structural & \multirow{2}*{COV-R $\uparrow$} & \multirow{2}*{COV-P $\uparrow$} & \multirow{2}*{\# Element $\downarrow$} & \multirow{2}*{$\rho$ $\downarrow$} & \multirow{2}*{$\mathcal{E}$ $\downarrow$}\\
  %  & & validity $\uparrow$ & validity $\uparrow$ & & & & & \\
  % \cline{1-9}
  % Compy val on two rows -->
  \multirow{2}*{Dataset} & \multirow{2}*{Method} & \multicolumn{2}{|c|}{Validity $\uparrow$} & \multicolumn{2}{|c|}{COV $\uparrow$} & \multicolumn{3}{|c|}{Property Statistics $\downarrow$} \\
  \cline{3-9}
   & & Compositional validity $\uparrow$ & Structural validity $\uparrow$ & COV-R $\uparrow$ & COV-P $\uparrow$ & \# Element $\downarrow$ & $\rho$ $\downarrow$ & $\mathcal{E}$ $\downarrow$\\
  \cline{1-9}

  % Perov
  \multirow{5}*{Perov-5} & FTCP & 54.24 & 0.24 & 0 & 0 & 0.6297 & 10.27 & 156.0 \\
  \cline{2-9}
   & G-SchNet & 98.79 & 99.92 & 0.18 & 0.23 & 0.0368 & 1.625 & 4.746 \\
  \cline{2-9}
   & P-G-SchNet & \textbf{99.13} & 79.63 & 0.56 & 0.41 & 0.4552 & 0.2755 & 1.388 \\
  \cline{2-9}
   & CDVAE & 98.59 & \textbf{100} & 99.45 & 98.46 & 0.0628 & 0.1258 & 0.0264 \\
  \cline{2-9}
   & SyMat & 97.40 & \textbf{100} & 99.68 & 98.64 \textbf{*} & 0.0177 & 0.1893 & 0.2364 \\
  \cline{2-9}
   & DiffCSP & 98.85 \textbf{*} & \textbf{100} & 99.74 \textbf{*} & 98.27 & 0.0128 & 0.111 & 0.0263 \\
  \cline{2-9}
   & Ours & 98.32 & \textbf{100} & \textbf{99.92} & \textbf{99.53} & \textbf{0.009} & \textbf{0.0826} & \textbf{0.0173} \\
  \cline{1-9}

  % Carbon
  \multirow{5}*{Carbon-24} & FTCP & - & 0.08 & 0 & 0 & - & 5.206 & 19.05 \\
  \cline{2-9}
   & G-SchNet & - & 99.94 & 0 & 0 & - & 0.9427 & 1.32 \\
  \cline{2-9}
   & P-G-SchNet & - & 48.39 & 0 & 0 & - & 1.533 & 134.7 \\
  \cline{2-9}
   & CDVAE & - & \textbf{100} & 99.8 & 83.08 & - & 0.1407 & 0.285 \\
  \cline{2-9}
   & SyMat & - & \textbf{100} & \textbf{99.9} & \textbf{97.59} & - & 0.1195 & 3.9576 \\
  \cline{2-9}
   & DiffCSP & - & \textbf{100} & \textbf{99.9} & 97.27 & - & 0.0805 & 0.082 \\
  \cline{2-9}
   & Ours & - & \textbf{100} & \textbf{99.9} & 85.63 & - & \textbf{0.043} &  \textbf{0.063} \\
  \cline{1-9}
 \end{tabularx}
 }
 \caption{The best performance is highlighted in bold.}
 \label{tbl-gen}
\end{table*}
% TABLE 2 END ------------>


% % TABLE 3 ------------>
% \begin{table*}
%   \centering
%     \setlength{\tabcolsep}{6 pt}
%     \renewcommand{\arraystretch}{1.2}
%  \begin{tabular}{ |c|c|c|c|c|c|c|c| }
%  \hline
%  % Header
%  \multirow{2}*{Method} & \multirow{2}*{\# of Samples} & \multicolumn{2}{|c|}{Perov-5}\\
%  \cline{3-4}
%   & & Match rate & RMSE \\
%  \hline

%   % CDVAE
%   \multirow{2}*{CDVAE} & 1 & 45.31 & 0.1138 \\
%   \cline{2-4}
%    & 20 & 88.51 & 0.0464 \\
%   \hline

%    % DiffCSP
%    \multirow{2}*{DiffCSP} & 1 & 52.02 & 0.076 \\
%   \cline{2-4}
%    & 20 & 98.6 & 0.0128 \\
%   \hline

%   % Ours (BERT)
%   \multirow{2}*{Ours (BERT)} & 1 & 94.58 & 0.0169 \\
%   \cline{2-4}
%    & 20 & 96.64 & 0.0109 \\
%   \hline

%   % Ours (T5)
%   \multirow{2}*{Ours (T5)} & 1 &  &   \\
%   \cline{2-4}
%    & 20 &  &   \\
%   \hline

%   % Ours (MatSciBERT)
%   \multirow{2}*{Ours (MatSciBERT)} & 1 & 95.24 & 0.0194 \\
%   \cline{2-4}
%    & 20 & 98.25 & 0.0085 \\
%   \hline

%  \end{tabular}
%    \caption{The best performance is highlighted in bold.}
%   \label{tbl-recons-encoders}
% \end{table*}
% % TABLE 3 END ------------>

% % TABLE 4 ------------>
% \begin{table*}
%   \centering
%     \setlength{\tabcolsep}{6 pt}
%     \renewcommand{\arraystretch}{1.2}
%  \begin{tabularx}{\textwidth}{ |c|c|X|X|X|X|X|X|X| }
%   \hline
%   % Header
%   \multirow{2}*{Dataset} & \multirow{2}*{Method} & \multicolumn{2}{|c|}{Validity ↑} & \multicolumn{2}{|c|}{COV ↑} & \multicolumn{3}{|c|}{Property Statistics ↓} \\
%   \cline{3-9}
%    & & \hspace{0pt} Compositional validity ↑ & Structural validity ↑ & COV-R ↑ & COV-P ↑ & \# Element EMD ↓ & Density EMD ↓ & Energy EMD ↓\\
%   \hline
%   \hline
%   % Perov
%   \multirow{6}*{Perov-5} & CDVAE & 98.59 & \textbf{100} & 99.45 & 98.46 & 0.0628 & 0.1258 & 0.0264 \\
%   \cline{2-9}
%    & SyMat & 97.4 & \textbf{100} & 99.68 & 98.64 & 0.0177 & 0.1893 & 0.2364 \\
%   \cline{2-9}
%    & DiffCSP & 98.85 & \textbf{100} & 99.74 & 98.27 & 0.0128 & 0.111 & \textbf{0.0263} \\
%   \cline{2-9}
%    & Ours (BERT) & 98.44 & 99.97 & 99.57 & 99.44 & 0.0148 & 0.0595 & - \\
%   \cline{2-9}
%    & Ours (T5) & 94.24 & 99.92 & 86.15 & 96.75 & 0.1090 & 0.3054 & - \\
%   \cline{2-9}
%    & Ours (MatSciBERT) & 98.32 & \textbf{100} & \textbf{99.92} & \textbf{99.53} & \textbf{0.009} & \textbf{0.0826} & - \\
%   \hline
%  \end{tabularx}
%  \caption{The best performance is highlighted in bold.}
%   \label{tbl-gen-encoders}
% \end{table*}
% % TABLE 4 END ------------>

% TABLE 5 ------------>
\begin{table*}
  \centering
    \setlength{\tabcolsep}{2.5 pt}
    \renewcommand{\arraystretch}{1.2}
    \scalebox{0.9}{
    \begin{tabular}{ |m{2in}|c|ccccc| } % angstrom symbol Å
 \cline{1-7}
 % Header
 % Chemical & Ground & \multirow{2}*{Sample 1} & \multirow{2}*{Sample 2} & \multirow{2}*{Sample 3} & \multirow{2}*{Sample 4} \\
 Description & Ground truth & \multicolumn{5}{c|}{Generated Samples} \\
 \cline{1-7}
 % \cline{1-6}
 
 % perov
  % HgCsO3
  CsO3Hg is (Cubic) Perovskite structured and crystallizes in the tetragonal P4mm space group. The structure consists of \dots
  % one Hg cluster inside a CsO3 framework. In the Hg cluster, Hg(1) is bonded in a 1-coordinate geometry to  atoms. In the CsO3 framework, Cs(1) is bonded to two equivalent O(2) and four equivalent O(1) atoms to form corner-sharing CsO6 octahedra. The corner-sharing octahedral tilt angles range from 0-1Å. Both Cs(1)-O(2) bond lengths are 2.23 Ã…. All Cs(1)-O(1) bond lengths are 2.23 Ã…. There are two inequivalent O sites. In the first O site, O(1) is bonded in a linear geometry to two equivalent Cs(1) atoms. In the second O site, O(2)
  is bonded in a linear geometry to two equivalent Cs(1) atoms. & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124_0.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124_1.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124_2.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124_3.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/14124_4.png}
  \end{minipage} \\
  \cline{1-7}
  
  % AuTaO2S
  TaAuSO2 crystallizes in the orthorhombic Pmm2 space group. Ta(1) is bonded to two equivalent S(1), \dots
  % two equivalent O(1), and two equivalent O(2) atoms to form distorted corner-sharing TaS2O4 octahedra. The corner-sharing octahedral tilt angles range from 0-51Â°. Both Ta(1)-S(1) bond lengths are 2.43 Ã…. Both Ta(1)-O(1) bond lengths are 2.19 Ã…. There is one shorter (1.83 Ã…) and one longer (2.55 Ã…) Ta(1)-O(2) bond length. Au(1) is bonded in a bent 120 degrees geometry to two equivalent S(1) atoms. Both Au(1)-S(1) bond lengths are 2.41 Ã…. S(1) is bonded in a 4-coordinate geometry to two equivalent Ta(1) and two equivalent Au(1) atoms. There are two inequivalent O sites. In the first O site, O(1) is bonded in a linear geometry to two equivalent Ta(1) atoms.
  In the second O site, O(2) is bonded in a distorted linear geometry to two equivalent Ta(1) atoms. & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778_0.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778_1.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778_2.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778_3.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/10778_4.png}
  \end{minipage} \\
  \cline{1-7}
  
  % AsYON2
  YN2OAs is alpha Rhenium trioxide-derived structured and crystallizes in the tetragonal P4mm space group. The structure \dots
  % consists of one As cluster inside a YN2O framework. In the As cluster, As(1) is bonded in a 1-coordinate geometry to  atoms. In the YN2O framework, Y(1) is bonded to four equivalent N(1) and two equivalent O(1) atoms to form corner-sharing YN4O2 octahedra. The corner-sharing octahedral tilt angles range from 0-1Â°. All Y(1)-N(1) bond lengths are 2.19 Ã…. There is one shorter (2.19 Ã…) and one longer (2.20 Ã…) Y(1)-O(1) bond length. N(1) is bonded in a linear geometry to two equivalent Y(1) atoms.
  O(1) is bonded in a linear geometry to two equivalent Y(1) atoms. & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558_0.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558_1.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558_2.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558_3.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/perov_samples/5558_4.png}
  \end{minipage} \\
  \cline{1-7}
  % \cline{1-6}

  % carbon
  % C14
  C crystallizes in the monoclinic Pm space group. There are fourteen inequivalent C sites. \dots
  % In the first C site, C(1) is bonded to one C(11), one C(9), and two equivalent C(14) atoms to form corner-sharing CC4 tetrahedra. The C(1)-C(11) bond length is 1.46 Å. The C(1)-C(9) bond length is 1.48 Å. Both C(1)-C(14) bond lengths are 1.54 Å. In the second C site, C(2) is bonded in a trigonal planar geometry to one C(6), one C(8), and one C(9) atom. The C(2)-C(6) bond length is 1.53 Ã…. The C(2)-C(8) bond length is 1.63 Ã…. The C(2)-C(9) bond length is 1.43 Ã…. In the third C site, C(3) is bonded to one C(13), one C(5), and two equivalent C(7) atoms to form corner-sharing CC4 tetrahedra. The C(3)-C(13) bond length is 1.43 Ã…. The C(3)-C(5) bond length is 1.42 Ã…. Both C(3)-C(7) bond lengths are 1.53 Ã…. In the fourth C site, C(4) is bonded to one C(14), one C(7), and two equivalent C(6) atoms to form corner-sharing CC4 tetrahedra. The C(4)-C(14) bond length is 1.60 Ã…. The C(4)-C(7) bond length is 1.46 Ã…. Both C(4)-C(6) bond lengths are 1.57 Ã…. In the fifth C site, C(5) is bonded in a trigonal planar geometry to one C(3), one C(8), and one C(9) atom. The C(5)-C(8) bond length is 1.54 Ã…. The C(5)-C(9) bond length is 1.39 Ã…. In the sixth C site, C(6) is bonded to one C(13), one C(2), and two equivalent C(4) atoms to form corner-sharing CC4 tetrahedra. The C(6)-C(13) bond length is 1.41 Ã…. In the seventh C site, C(7) is bonded to one C(12), one C(4), and two equivalent C(3) atoms to form corner-sharing CC4 tetrahedra. The C(7)-C(12) bond length is 1.55 Ã…. In the eighth C site, C(8) is bonded to one C(2), one C(5), and two equivalent C(10) atoms to form corner-sharing CC4 tetrahedra. Both C(8)-C(10) bond lengths are 1.55 Ã…. In the ninth C site, C(9) is bonded in a trigonal planar geometry to one C(1), one C(2), and one C(5) atom. In the tenth C site, C(10) is bonded to one C(12), one C(14), and two equivalent C(8) atoms to form corner-sharing CC4 tetrahedra. The C(10)-C(12) bond length is 1.49 Ã…. The C(10)-C(14) bond length is 1.56 Ã…. In the eleventh C site, C(11) is bonded to one C(1), one C(13), and two equivalent C(12) atoms to form corner-sharing CC4 tetrahedra. The C(11)-C(13) bond length is 1.46 Ã…. Both C(11)-C(12) bond lengths are 1.52 Ã…. In the twelfth C site, C(12) is bonded to one C(10), one C(7), and two equivalent C(11) atoms to form corner-sharing CC4 tetrahedra. In the thirteenth C site, C(13) is bonded in a distorted trigonal planar geometry to one C(11), one C(3), and one C(6) atom. In the fourteenth C site, C(14) is 
  bonded to one C(10), one C(4), and two equivalent C(1) atoms to form corner-sharing CC4 tetrahedra. & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49_0.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49_1.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49_2.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49_3.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-92144-1112-49_4.png}
  \end{minipage} \\
  \cline{1-7}
  
  % C6
  C crystallizes in the orthorhombic Fmmm space group. There are two inequivalent C sites. In the first C site, \dots
  % C(1) is bonded to one C(2) and three equivalent C(1) atoms to form a mixture of corner and edge-sharing CC4 trigonal pyramids. The C(1)-C(2) bond length is 1.52 Å. There are two shorter (1.52 Å) and one longer (1.56 Å) C(1)-C(1) bond length. In the second C site, C(2) is bonded to two equivalent C(1) and two equivalent C(2) atoms to form corner-sharing CC4 tetrahedra.
  Both C(2)-C(2) bond lengths are 1.53 Å. & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45_0.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45_1.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45_2.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45_3.png}
  \end{minipage} & \begin{minipage}{.1\linewidth}
      \includegraphics[width=\linewidth]{Images/carbon_samples/C-53844-8150-45_4.png}
  \end{minipage} \\
  \cline{1-7}
 \end{tabular}
 }
   \caption{Samples from text description only}
  \label{tbl-samples}
\end{table*}
% TABLE 5 END ------------>

% ---------------figs--------------- %
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{Images/runtime4.png}
	\caption{Match rate vs running time for different timesteps}
	\label{fig:text}
\end{figure}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=\columnwidth]{Images/runtime_perov_5.png}
% 	\caption{Match rate vs running time for different timesteps for the Perov-5 dataset}
% 	\label{fig:text}
% \end{figure}

% \begin{figure}
% 	\centering
% 	\includegraphics[width=\columnwidth]{Images/runtime_carbon_24.png}
% 	\caption{Match rate vs running time for different timesteps for the Carbon-24 dataset}
% 	\label{fig:text}
% \end{figure}

